Model Assertions for Monitoring and Improving ML Models

ML models are increasingly deployed in settings with real world interactions such as vehicles, but unfortunately, these models can fail in systematic ways. To prevent errors, ML engineering teams monitor and continuously improve these models. We propose a new abstraction, model assertions, that adapts the classical use of program assertions as a way to monitor and improve ML models. Model assertions are arbitrary functions over a model's input and output that indicate when errors may be occurring, e.g., a function that triggers if an object rapidly changes its class in a video. We propose methods of using model assertions at all stages of ML system deployment, including runtime monitoring, validating labels, and continuously improving ML models. For runtime monitoring, we show that model assertions can find high confidence errors, where a model returns the wrong output with high confidence, which uncertainty-based monitoring techniques would not detect. For training, we propose two methods of using model assertions. First, we propose a bandit-based active learning algorithm that can sample from data flagged by assertions and show that it can reduce labeling costs by up to 40% over traditional uncertainty-based methods. Second, we propose an API for generating "consistency assertions" (e.g., the class change example) and weak labels for inputs where the consistency assertions fail, and show that these weak labels can improve relative model quality by up to 46%. We evaluate model assertions on four real-world tasks with video, LIDAR, and ECG data.

==> tex/background.tex <==
\section{Background and Motivation}
\label{sec:background}


\minihead{Deployment of real-world ML systems}
In discussion with industry partners, we have found that real-world ML systems
feature two unique properties.

First, these models are deployed on orders of magnitude more data than can
possibly be labeled, so a labeled sample cannot capture all deployment
conditions. For example:
\begin{itemize}[leftmargin=1em]
  \item \textbf{Video analytics}: many modern video analytics
  systems~\cite{kang2017noscope, kang2018blazeit, hsieh2018focus,
  jiang2018chameleon, xu2019vstore, canel2019scaling} use object detection
  methods (i.e., methods for detecting the location and object class in an image
  or frame of video) that were developed by other academic
  labs~\cite{he2017mask, redmon2017yolo9000}. These object detection methods
  were trained on \emph{still image data}, despite being deployed on video:
  collecting labels over video is extremely costly, so these models were
  pretrained on publicly available datasets~\cite{lin2014microsoft}. Thus, the
  training set is not representative of the deployment set.

  \item \textbf{Autonomous vehicles:} under mild assumptions, the Tesla fleet of
  vehicles will see over 100$\times$ more images in a day than in the largest
  existing image dataset~\cite{sun2017revisiting}. Furthermore, random data
  collection might miss important data points. Pedestrians will normally not be
  dressed in Halloween costumes, except on Halloween, which is 1/365 of the
  deployment data. In Tempe, Arizona, where Uber's autonomous vehicles were
  deployed, it generally does not snow. Collecting data in Tempe will not be
  representative of Alaska.

  \item \textbf{ECG classification:} the largest ECG dataset labeled for
  arrhythmia (heart conditions) by ``two orders of magnitude'' contains 64,121
  samples of 30 seconds or around 534 hours~\cite{rajpurkar2017cardiologist}.
  The authors sampled these data points from a deployment setting of 300,000
  patients, who wore the ECG leads for about two weeks each, which is
  approximately 6 orders of magnitude more data. Furthermore, the model will be
  deployed on continuous data, not 30 second slices.

\end{itemize}


Second, ML deployments are incredibly complex and developed by teams of
specialists, so the domain experts who monitor ML models may not know how to fix
errors in deployment. For example, an autonomous vehicle might be developed by
sensor experts (e.g., hardware engineers), deep learning researchers, and site
reliability engineers (SREs). The hardware engineer might build a sensor. The
researchers might develop a model for detecting objects from a LIDAR
sensor~\cite{zhou2018voxelnet}. Then, a SRE might identify systematic errors in
an ML model, e.g., aberrant behavior in rain, but may not be an expert in ML
model development. As a result, it is critical for different teams to be able to
collaborate in monitoring these deployments.



\minihead{Robustness and verification of ML models}
As ML models are deployed in mission-critical settings, they would ideally be
formally verified. However, a formal specification may not even be possible for
real-world deployments. In real-world deployments, even humans may be unable to
distinguish a car from a truck at a distance. Furthermore, the largest verified
models we are aware of verify simple properties (e.g., given an object location
and velocity, avoid the object) and are orders of magnitude smaller than the
networks we consider~\cite{wang2018formal, sun2019formal, katz2017reluplex}.


Researchers have also proposed studying the statistical robustness of ML
models~\cite{wong2018scaling, steinhardt2017certified, steinhardt2018robust}.
However, the robustness guarantees are only with respect to small perturbations,
such as small $L_{\infty}$ or $L_2$ pixel-level differences for
images~\cite{cohen2019certified, raghunathan2018certified}. These perturbations
do not capture real-world transforms, such as rotations, which are known to fool
state-of-the-art vision models~\cite{engstrom2017rotation}. We are unaware of
any robustness guarantees outside of these simple perturbations.



\minihead{Existing solutions for ML QA}
Existing solutions focus on training pipelines~\cite{renggli2019continuous}, on
schema validation~\cite{polyzotis2019data, baylor2017tfx}, or ad-hoc, domain
specific checks~\cite{jin2018unsupervised}. As we have discussed,
training/validation set accuracy may not represent all situations, so
solutions that focus on training are insufficient. In schema validation, inputs
to models are validated to ensure they fall in valid ranges, e.g., a Boolean
feature to an ML model should not have a value of 10. Schema validation does not
work for the real-world, unstructured data sources (e.g., image pixels) for
which deep learning is most successful. Finally, ad-hoc and domain specific
checks must be implemented for every new domain.


==> tex/design.tex <==
\section{\sn System Design}
\label{sec:design}

To evaluate the utility of model assertions across a range of domains, we built
\sn, a prototype library for deploying model assertions.


\begin{figure}
  \includegraphics[width=0.99\columnwidth]{figures/omg-system-diagram.png}
  \vspace{-0.5em}
  \caption{A system diagram for \sn. Domain experts and users will create
  model assertions, which will be registered in an assertion database. These
  assertions will be executed over model deployment and, when triggered, can be
  used to monitor statistics of failures or to collect data. The collected data
  can be used to further train the ML model, via active learning or weak
  supervision.}
  \label{fig:omg-sys}
\end{figure}


\minihead{Overview}
\sn consists of four components: an assertion database, an execution environment
(for the batch and streaming settings), a data collection component, and a
retraining component. We describe the components in detail below and show a
system diagram in Figure~\ref{fig:omg-sys}.

An important feature of \sn is that it integrates with existing ML deployment
pipeline with only a series of callbacks. In discussions with industry partners,
we have found that production ML deployments continuously collect data and train
models~\cite{karpathy2018building}. \sn could be inserted into these existing
pipelines. In our evaluation, we deployed \sn with no changes to the core
training or inference code (several periphery changes were required, such as
removing hard coded data paths).


\minihead{Model assertion database}
The model assertion database allows domain experts to collaborative add model
assertions. Currently, \sn has a different database per task and model.

Model assertions are registered as functions that take as input model inputs and
outputs. Concretely, suppose an assertion were for an object
detection model in video. The input is a sequence of frames and the output is a
set of bounding boxes for each frame. A user could write an assertion for
detecting flickering, which would have Python3 signature:
\begin{lstlisting}
  def flickering(List[PixelBuf] recent_frames,
    List[BoundingBox] recent_ouputs) -> Float
\end{lstlisting}
A second user could write an assertion to catch when objects highly overlap in
incorrect ways. Once these assertions are registered, they can be used by any
user.


\minihead{Execution environment}
After model assertions are registered in the database, \sn can execute these
assertions in existing model deployment systems by adding a call to \sn's
execution engine. At deployment, \sn simply takes in model inputs and outputs
and executes user-selected model assertions. By only requiring the inputs and
outputs, the core inference code does not need to be modified.

By default, \sn will only log the number of times an assertion was triggered, as
collecting model inputs can be expensive. If desired, the user can write a
callback to perform an action when an assertion is triggered. For example, the
system may raise an alert if the severity score is above some threshold.

In a streaming setting, as the model runs, the execution environment keeps state
to track the current input and output of the model, along with a limited number
of recent inputs. After the model makes a prediction, the state is passed to
each assertion callback.


\minihead{Data collection}
Many production ML systems continuously collect new data for labeling to further
train ML models~\cite{karpathy2018building}. Many ML systems are unable to
collect all input data due to data volumes, e.g., billions of images per day in
an autonomous vehicle fleet.

As we show, model assertions can be used as a signal to decide which data points
to select (Section~\ref{sec:eval}). In \sn, we implement a data collection
procedure based on model assertions for the batch setting, i.e., over historical
data. As described in full in Section~\ref{sec:alg}, \sn will select points
based on a bandit algorithm. To implement data collection, \sn requires access
to a callback that will label a given data point.



\minihead{Retraining component}
As data that has triggered model assertions is collected and labeled, \sn can
continuously train ML models. \sn simply requires access to the training
pipeline and will update the data inputs. The user need not change any core
training code.

Furthermore, certain assertions can be paired with corrective rules that propose
corrected labels. These corrected labels can be used to train the model with no
human input as a form of weak supervision. Currently, \sn will update the labels
for existing data, but it could be integrated with existing weak supervision
pipelines~\cite{ratner2017weak, varma2018reef}.

